Weakly-supervised Caricature Face Parsing through Domain Adaptation

A caricature is an artistic form of a person's picture in which certain striking characteristics are abstracted or exaggerated in order to create a humor or sarcasm effect. For numerous caricature related applications such as attribute recognition and caricature editing, face parsing is an essential pre-processing step that provides a complete facial structure understanding. However, current state-of-the-art face parsing methods require large amounts of labeled data on the pixel-level and such process for caricature is tedious and labor-intensive. For real photos, there are numerous labeled datasets for face parsing. Thus, we formulate caricature face parsing as a domain adaptation problem, where real photos play the role of the source domain, adapting to the target caricatures. Specifically, we first leverage a spatial transformer based network to enable shape domain shifts. A feed-forward style transfer network is then utilized to capture texture-level domain gaps. With these two steps, we synthesize face caricatures from real photos, and thus we can use parsing ground truths of the original photos to learn the parsing model. Experimental results on the synthetic and real caricatures demonstrate the effectiveness of the proposed domain adaptation algorithm. Code is available at: https://github.com/ZJULearning/CariFaceParsing .

==> egbib.tex <==
\textit{}@STRING{TPAMI	= "IEEE Transactions on Pattern Analysis and Machine Intelligence"}
@STRING{IJCV	= "International Journal of Computer Vision"}
@STRING{TIP	= "IEEE Transactions on Image Processing"}
@STRING{TIT	= "IEEE Transactions on Information Theory"}
@STRING{TMM	= "IEEE Transactions on Multimedia"}
@STRING{TCSVT	= "IEEE Transactions on Circuits and Systems for Video Technology"}
@STRING{TSP	= "IEEE Transactions on Signal Processing"}
@STRING{CVIU	= "Computer Vision and Image Understanding"}
@STRING{PR		= "Pattern Recognition"}
@STRING{JMLR	= "Journal of Machine Learning Research"}
@STRING{TOG		= "ACM Transactions on Graphics (Proceedings of SIGGRAPH)"}
@STRING{TOGA	= "ACM Transactions on Graphics (Proceedings of SIGGRAPH Asia)"}

@STRING{PAKDD	= "Pacific-Asia Conference on Knowledge Discovery and Data Mining"}
@STRING{IJCAI	= "International Joint Conference on Artificial Intelligence"}
@STRING{AAAI	= "AAAI Conference on Artificial Intelligence"}
@STRING{NIPS	= "Neural Information Processing Systems"}
@STRING{CVPR	= "IEEE Conference on Computer Vision and Pattern Recognition"}
@STRING{CVPRW	= "IEEE Conference on Computer Vision and Pattern Recognition Workshops"}
@STRING{ECCV	= "European Conference on Computer Vision"}
@STRING{ACCV	= "Asia Conference on Computer Vision"}
@STRING{ICCV	= "IEEE International Conference on Computer Vision"}
@STRING{ICIP	= "IEEE International Conference on Image Processing"}
@STRING{ICCP	= "IEEE International Conference on Computational Photography"}
@STRING{ICML	= "International Conference on Machine Learning"}
@STRING{BMVC	= "British Machine Vision Conference"}
@STRING{ACMMM	= "ACM International conference on Multimedia"}
@STRING{Arxiv	= "Arxiv"}
@STRING{ICPR 	= "International Conference on Pattern Recognition"}
@STRING{ICME 	= "IEEE International Conference on Multimedia and Expo"}
@STRING{VMV	= "Vision, Modelling and Visualization"}
@STRING{ICASSP	= "IEEE International Conference on Acoustics, Speech, and Signal Processing"}
@STRING{ICLR	= "International Conference on Learning Representations"}



@InProceedings{C2,
	author = 	 "Jones, C.D. and Smith, A.B. and Roberts, E.F.",
	title =        "Article Title",
	booktitle =        "Proceedings Title",
	organization = "IEEE",
	year = 	 "2003",
	volume = 	 "II",
	pages = 	 "803-806"
}

@Article{Lamp86,
	author =       "A.B. Smith and C.D. Jones and E.F. Roberts",
	title =        "Article Title",
	journal = 	 "Journal",
	year = 	 "1920",
	volume = 	 "62",
	pages = 	 "291-294",
	month = 	 "January"
}

// knowledge transfer


@inproceedings{gong2012geodesic,
	title={Geodesic flow kernel for unsupervised domain adaptation},
	author={Gong, Boqing and Shi, Yuan and Sha, Fei and Grauman, Kristen},
	booktitle={CVPR},
	pages={2066--2073},
	year={2012},
	organization={IEEE}
}

@inproceedings{long2015learning,
	title={Learning transferable features with deep adaptation networks},
	author={Long, Mingsheng and Cao, Yue and Wang, Jianmin and Jordan, Michael I},
	booktitle={ICML},
	year={2015}
}

@article{ganin2016domain,
	title={Domain-adversarial training of neural networks},
	author={Ganin, Yaroslav and Ustinova, Evgeniya and Ajakan, Hana and Germain, Pascal and Larochelle, Hugo and Laviolette, Fran{\c{c}}ois and Marchand, Mario and Lempitsky, Victor},
	journal={JMLR},
	volume={17},
	number={1},
	pages={2096--2030},
	year={2016},
	publisher={JMLR. org}
}

@inproceedings{rashid2017interspecies,
	title={Interspecies knowledge transfer for facial keypoint detection},
	author={Rashid, Maheen and Gu, Xiuye and Jae Lee, Yong},
	booktitle={CVPR},
	pages={6894--6903},
	year={2017}
}

@article{hoffman2016fcns,
	title={Fcns in the wild: Pixel-level adversarial and constraint-based adaptation},
	author={Hoffman, Judy and Wang, Dequan and Yu, Fisher and Darrell, Trevor},
	journal={arXiv preprint arXiv:1612.02649},
	year={2016}
}

@inproceedings{chen2017no,
	title={No more discrimination: Cross city adaptation of road scene segmenters},
	author={Chen, Yi-Hsin and Chen, Wei-Yu and Chen, Yu-Ting and Tsai, Bo-Cheng and Frank Wang, Yu-Chiang and Sun, Min},
	booktitle={ICCV},
	pages={1992--2001},
	year={2017}
}

@inproceedings{hoffman2017cycada,
	title={Cycada: Cycle-consistent adversarial domain adaptation},
	author={Hoffman, Judy and Tzeng, Eric and Park, Taesung and Zhu, Jun-Yan and Isola, Phillip and Saenko, Kate and Efros, Alexei A and Darrell, Trevor},
	booktitle={ICML},
	year={2018}
}

@inproceedings{tsai2018learning,
	title={Learning to adapt structured output space for semantic segmentation},
	author={Tsai, Yi-Hsuan and Hung, Wei-Chih and Schulter, Samuel and Sohn, Kihyuk and Yang, Ming-Hsuan and Chandraker, Manmohan},
	booktitle={CVPR},
	year={2018}
}

@inproceedings{pan2018two,
	title={Two at once: Enhancing learning and generalization capacities via ibn-net},
	author={Pan, Xingang and Luo, Ping and Shi, Jianping and Tang, Xiaoou},
	booktitle={ECCV},
	pages={464--479},
	year={2018}
}

//face parsing
@inproceedings{luo2012hierarchical,
	title={Hierarchical face parsing via deep learning},
	author={Luo, Ping and Wang, Xiaogang and Tang, Xiaoou},
	booktitle={CVPR},
	pages={2480--2487},
	year={2012},
	organization={IEEE}
}

@inproceedings{smith2013exemplar,
	title={Exemplar-based face parsing},
	author={Smith, Brandon M and Zhang, Li and Brandt, Jonathan and Lin, Zhe and Yang, Jianchao},
	booktitle={CVPR},
	pages={3484--3491},
	year={2013}
}

@inproceedings{liu2015multi,
	title={Multi-objective convolutional learning for face labeling},
	author={Liu, Sifei and Yang, Jimei and Huang, Chang and Yang, Ming-Hsuan},
	booktitle={CVPR},
	pages={3451--3459},
	year={2015}
}

@inproceedings{jackson2016cnn,
	title={A CNN cascade for landmark guided semantic part segmentation},
	author={Jackson, Aaron S and Valstar, Michel and Tzimiropoulos, Georgios},
	booktitle={ECCV},
	pages={143--155},
	year={2016},
	organization={Springer}
}

@inproceedings{zhao2017pyramid,
	title={Pyramid scene parsing network},
	author={Zhao, Hengshuang and Shi, Jianping and Qi, Xiaojuan and Wang, Xiaogang and Jia, Jiaya},
	booktitle={IEEE Conf. on Computer Vision and Pattern Recognition (CVPR)},
	pages={2881--2890},
	year={2017}
}

@inproceedings{Liu2017FacePV,
	title={Face Parsing via Recurrent Propagation},
	author={Sifei Liu and Jianping Shi and Liang Ji and Ming-Hsuan Yang},
	booktitle={BMVC},
	year={2017},
	volume={abs/1708.01936}
}

@inproceedings{wei2017learning,
	title={Learning adaptive receptive fields for deep image parsing network},
	author={Wei, Zhen and Sun, Yao and Wang, Jinqiao and Lai, Hanjiang and Liu, Si},
	booktitle={CVPR},
	pages={2434--2442},
	year={2017}
}

//gan





@inproceedings{goodfellow2014generative,
	title={Generative adversarial nets},
	author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
	booktitle={NIPS},
	year={2014}
}

@inproceedings{arjovsky2017wasserstein,
	title={Wasserstein generative adversarial networks},
	author={Arjovsky, Martin and Chintala, Soumith and Bottou, L{\'e}on},
	booktitle={ICML},
	year={2017}
}


// style transfer


@article{reinhard2001color,
	title={Color transfer between images},
	author={Reinhard, Erik and Adhikhmin, Michael and Gooch, Bruce and Shirley, Peter},
	journal={IEEE Computer graphics and applications},
	volume={21},
	number={5},
	pages={34--41},
	year={2001},
	publisher={IEEE}
}

@inproceedings{pitie2005n,
	title={N-dimensional probablility density function transfer and its application to colour transfer},
	author={Pitie, Francois and Kokaram, Anil C and Dahyot, Rozenn},
	booktitle={ICCV},
	year={2005},
	organization={IEEE}
}

@inproceedings{freedman2010object,
	title={Object-to-object color transfer: Optimal flows and smsp transformations},
	author={Freedman, Daniel and Kisilev, Pavel},
	booktitle={CVPR},
	year={2010},
	organization={IEEE}
}

@article{shih2013data,
	title={Data-driven hallucination of different times of day from a single outdoor photo},
	author={Shih, Yichang and Paris, Sylvain and Durand, Fr{\'e}do and Freeman, William T},
	journal={TOG},
	volume={32},
	number={6},
	pages={200},
	year={2013},
	publisher={ACM}
}

@article{shih2014style,
	title={Style transfer for headshot portraits},
	author={Shih, YiChang and Paris, Sylvain and Barnes, Connelly and Freeman, William T and Durand, Fr{\'e}do},
	journal={TOG},
	volume={33},
	number={4},
	pages={148},
	year={2014},
	publisher={ACM}
}


@article{tsai2016sky,
	title={Sky is not the limit: semantic-aware sky replacement.},
	author={Tsai, Yi-Hsuan and Shen, Xiaohui and Lin, Zhe and Sunkavalli, Kalyan and Yang, Ming-Hsuan},
	journal={TOG},
	volume={35},
	number={4},
	pages={149--1},
	year={2016}
}

@inproceedings{gatys2015texture,
	title={Texture synthesis using convolutional neural networks},
	author={Gatys, Leon and Ecker, Alexander S and Bethge, Matthias},
	booktitle={NIPS},
	year={2015}
}

@inproceedings{gatys2016image,
	title={Image style transfer using convolutional neural networks},
	author={Gatys, Leon A and Ecker, Alexander S and Bethge, Matthias},
	booktitle={CVPR},
	year={2016}
}

@inproceedings{li2016combining,
	title={Combining markov random fields and convolutional neural networks for image synthesis},
	author={Li, Chuan and Wand, Michael},
	booktitle={CVPR},
	year={2016}
}

@inproceedings{johnson2016perceptual,
	title={Perceptual losses for real-time style transfer and super-resolution},
	author={Johnson, Justin and Alahi, Alexandre and Fei-Fei, Li},
	booktitle={ECCV},
	year={2016},
}

@inproceedings{li2017diversified,
	title={Diversified texture synthesis with feed-forward networks},
	author={Li, Yijun and Fang, Chen and Yang, Jimei and Wang, Zhaowen and Lu, Xin and Yang, Ming-Hsuan},
	booktitle={CVPR},
	year={2017}
}

@inproceedings{chen2017stylebank,
	title={Stylebank: An explicit representation for neural image style transfer},
	author={Chen, Dongdong and Yuan, Lu and Liao, Jing and Yu, Nenghai and Hua, Gang},
	booktitle={CVPR},
	year={2017}
}

@inproceedings{huang2017arbitrary,
	title={Arbitrary Style Transfer in Real-Time with Adaptive Instance Normalization.},
	author={Huang, Xun and Belongie, Serge J},
	booktitle={ICCV},
	year={2017}
}

@article{liao2017visual,
	title={Visual attribute transfer through deep image analogy},
	author={Liao, Jing and Yao, Yuan and Yuan, Lu and Hua, Gang and Kang, Sing Bing},
	journal={TOG},
	volume={36},
	number={4},
	pages={120},
	year={2017},
	publisher={ACM}
}

@inproceedings{li2017demystifying,
	title={Demystifying neural style transfer},
	author={Li, Yanghao and Wang, Naiyan and Liu, Jiaying and Hou, Xiaodi},
	booktitle={IJCAI},
	year={2017}
}

@inproceedings{li2017universal,
	title={Universal style transfer via feature transforms},
	author={Li, Yijun and Fang, Chen and Yang, Jimei and Wang, Zhaowen and Lu, Xin and Yang, Ming-Hsuan},
	booktitle={NIPS},
	year={2017}
}

@inproceedings{li2018closed,
	title={A closed-form solution to photorealistic image stylization},
	author={Li, Yijun and Liu, Ming-Yu and Li, Xueting and Yang, Ming-Hsuan and Kautz, Jan},
	booktitle={ECCV},
	year={2018}
}

@inproceedings{reed2016generative,
	title={Generative adversarial text to image synthesis},
	author={Reed, Scott and Akata, Zeynep and Yan, Xinchen and Logeswaran, Lajanugen and Schiele, Bernt and Lee, Honglak},
	booktitle={ICML},
	year={2016}
}

@inproceedings{ledig2017photo,
	title={Photo-Realistic Single Image Super-Resolution Using a Generative Adversarial Network.},
	author={Ledig, Christian and Theis, Lucas and Husz{\'a}r, Ferenc and Caballero, Jose and Cunningham, Andrew and Acosta, Alejandro and Aitken, Andrew P and Tejani, Alykhan and Totz, Johannes and Wang, Zehan and others},
	booktitle={CVPR},
	year={2017}
}

@inproceedings{vondrick2016generating,
	title={Generating videos with scene dynamics},
	author={Vondrick, Carl and Pirsiavash, Hamed and Torralba, Antonio},
	booktitle={NIPS},
	year={2016}
}

@inproceedings{shrivastava2017learning,
	title={Learning from Simulated and Unsupervised Images through Adversarial Training.},
	author={Shrivastava, Ashish and Pfister, Tomas and Tuzel, Oncel and Susskind, Joshua and Wang, Wenda and Webb, Russell},
	booktitle={CVPR},
	year={2017}
}


// image translation


@inproceedings{isola2017image,
	title={Image-to-Image Translation with Conditional Adversarial Networks},
	author={Isola, Phillip and Zhu, Jun-Yan and Zhou, Tinghui and Efros, Alexei A},
	booktitle={CVPR},
	year={2017},
}



@inproceedings{kim2017learning,
	title={Learning to discover cross-domain relations with generative adversarial networks},
	author={Kim, Taeksoo and Cha, Moonsu and Kim, Hyunsoo and Lee, Jung Kwon and Kim, Jiwon},
	booktitle={ICML},
	year={2017}
}

@inproceedings{zhu2017unpaired,
	title={Unpaired image-to-image translation using cycle-consistent adversarial networks},
	author={Zhu, Jun-Yan and Park, Taesung and Isola, Phillip and Efros, Alexei A},
	booktitle={ICCV},
	year={2017}
}


@inproceedings{liu2017unsupervised,
	title={Unsupervised image-to-image translation networks},
	author={Liu, Ming-Yu and Breuel, Thomas and Kautz, Jan},
	booktitle={NIPS},
	year={2017}
}

@inproceedings{zhu2017toward,
	title={Toward multimodal image-to-image translation},
	author={Zhu, Jun-Yan and Zhang, Richard and Pathak, Deepak and Darrell, Trevor and Efros, Alexei A and Wang, Oliver and Shechtman, Eli},
	booktitle={NIPS},
	year={2017}
}

@inproceedings{wang2017high,
	title={High-resolution image synthesis and semantic manipulation with conditional gans},
	author={Wang, Ting-Chun and Liu, Ming-Yu and Zhu, Jun-Yan and Tao, Andrew and Kautz, Jan and Catanzaro, Bryan},
	booktitle={CVPR},
	year={2018},
}


@inproceedings{choi2017stargan,
	title={Stargan: Unified generative adversarial networks for multi-domain image-to-image translation},
	author={Choi, Yunjey and Choi, Minje and Kim, Munyoung and Ha, Jung-Woo and Kim, Sunghun and Choo, Jaegul},
	booktitle={CVPR},
	year={2018}
}

@inproceedings{DRIT,
	author = {Lee, Hsin-Ying and Tseng, Hung-Yu and Huang, Jia-Bin and Singh, Maneesh Kumar and Yang, Ming-Hsuan},
	booktitle = {ECCV},
	title = {Diverse Image-to-Image Translation via Disentangled Representations},
	year = {2018}
}

@inproceedings{huang2018multimodal,
	title={Multimodal Unsupervised Image-to-Image Translation},
	author={Huang, Xun and Liu, Ming-Yu and Belongie, Serge and Kautz, Jan},
	booktitle = {ECCV},
	year={2018}
}

//caricatures

@inproceedings{akleman2000making,
	title={Making extreme caricatures with a new interactive 2D deformation technique with simplicial complexes},
	author={Akleman, Ergun and Palmer, James and Logan, Ryan},
	booktitle={Proceedings of Visual},
	year={2000}
}

@inproceedings{luo2002exaggeration,
	title={Exaggeration of facial features in caricaturing},
	author={Luo, Wan Chi and Liu, Pin Chou and Ouhyoung, Ming},
	booktitle={Proc. Int. Computer Symposium},
	year={2002}
}

@inproceedings{liao2004automatic,
	title={Automatic caricature generation by analyzing facial features},
	author={Liao, Pei-Ying Chiang Wen-Hung and Li, Tsai-Yen},
	booktitle={ACCV},
	year={2004}
}

@article{zheng2017photo,
	title={Photo-to-caricature translation on faces in the wild},
	author={Zheng, Ziqiang and Zheng, Haiyong and Yu, Zhibin and Gu, Zhaorui and Zheng, Bing},
	journal={arXiv preprint arXiv:1711.10735},
	year={2017}
}

@article{cao2018carigans,
	title={CariGANs: Unpaired Photo-to-Caricature Translation},
	author={Cao, Kaidi and Liao, Jing and Yuan, Lu},
	journal={arXiv preprint arXiv:1811.00222},
	year={2018}
}

@article{li2018carigan,
	title={CariGAN: Caricature Generation through Weakly Paired Adversarial Learning},
	author={Li, Wenbin and Xiong, Wei and Liao, Haofu and Huo, Jing and Gao, Yang and Luo, Jiebo},
	journal={arXiv preprint arXiv:1811.00445},
	year={2018}
}

// dataset

@inproceedings{HuoBMVC2018WebCaricature,
	author    = {Jing Huo and
	Wenbin Li and
	Yinghuan Shi and
	Yang Gao and
	Hujun Yin},
	title     = {WebCaricature: a benchmark for caricature recognition},
	booktitle={BMVC},
	year      = {2018}
}

// toolbox

@article{paszke2017automatic,
	title={Automatic differentiation in pytorch},
	author={Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
	year={2017}
}

// deep learning

@inproceedings{krizhevsky2012imagenet,
	title={Imagenet classification with deep convolutional neural networks},
	author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
	booktitle={NIPS},
	year={2012}
}

@inproceedings{simonyan2014very,
	title={Very deep convolutional networks for large-scale image recognition},
	author={Simonyan, Karen and Zisserman, Andrew},
	booktitle={ICLR},
	year={2015}
}

@inproceedings{szegedy2015going,
	title={Going deeper with convolutions},
	author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
	booktitle={CVPR},
	year={2015}
}

@inproceedings{he2016deep,
	title={Deep residual learning for image recognition},
	author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
	booktitle={CVPR},
	year={2016}
}

@inproceedings{huang2017densely,
	title={Densely connected convolutional networks.},
	author={Huang, Gao and Liu, Zhuang and Van Der Maaten, Laurens and Weinberger, Kilian Q},
	booktitle={CVPR},
	year={2017}
}

@inproceedings{kingma2014adam,
	title={Adam: A method for stochastic optimization},
	author={Kingma, Diederik P and Ba, Jimmy},
	booktitle={ICLR},
	year={2015}
}

// stn

@inproceedings{jaderberg2015spatial,
	title={Spatial transformer networks},
	author={Jaderberg, Max and Simonyan, Karen and Zisserman, Andrew and kavukcuoglu, koray},
	booktitle={NIPS},
	year={2015}
}

@inproceedings{ganin2016deepwarp,
	title={Deepwarp: Photorealistic image resynthesis for gaze manipulation},
	author={Ganin, Yaroslav and Kononenko, Daniil and Sungatullina, Diana and Lempitsky, Victor},
	booktitle={ECCV},
	year={2016},
}

@inproceedings{park2017transformation,
	title={Transformation-grounded image generation network for novel 3d view synthesis},
	author={Park, Eunbyung and Yang, Jimei and Yumer, Ersin and Ceylan, Duygu and Berg, Alexander C},
	booktitle={CVPR},
	year={2017},
}

@inproceedings{Wang_afrcnnCVPR2017,
	Author = {Xiaolong Wang and Abhinav Shrivastava and Abhinav Gupta},
	Title = {A-Fast-RCNN: Hard Positive Generation via Adversary for Object Detection},
	Booktitle = {CVPR},
	Year = {2017},
}

@inproceedings{wu2017recursive,
	title={Recursive spatial transformer (rest) for alignment-free face recognition},
	author={Wu, Wanglong and Kan, Meina and Liu, Xin and Yang, Yi and Shan, Shiguang and Chen, Xilin},
	booktitle={CVPR},
	year={2017}
}

@inproceedings{dai2017deformable,
	title={Deformable Convolutional Networks},
	author={Dai, Jifeng and Qi, Haozhi and Xiong, Yuwen and Li, Yi and Zhang, Guodong and Hu, Han and Wei, Yichen},
	booktitle={ICCV},
	year={2017}
}

@inproceedings{lin2018stgan,
	title={ST-GAN: Spatial Transformer Generative Adversarial Networks for Image Compositing},
	author={Lin, Chen-Hsuan and Yumer, Ersin and Wang, Oliver and Shechtman, Eli and Lucey, Simon},
	booktitle={CVPR},
	year={2018}
}

@inproceedings{xiao2018spatially,
	title={Spatially transformed adversarial examples},
	author={Xiao, Chaowei and Zhu, Jun-Yan and Li, Bo and He, Warren and Liu, Mingyan and Song, Dawn},
	booktitle={ICLR},
	year={2018}
}

@inproceedings{zhou2018gridface,
	title={GridFace: Face Rectification via Learning Local Homography Transformations},
	author={Zhou, Erjin and Cao, Zhimin and Sun, Jian},
	booktitle={ECCV},
	year={2018},
}

@inproceedings{Shu-ECCV18,
	title={Deforming Autoencoders: Unsupervised Disentangling of Shape and Appearance},
	author={Zhixin Shu and Mir Sahasrabudhe and Riza Alp Guler and Dimitris Samaras and Nikos Paragios and Iasonas Kokkinos},
	booktitle={ECCV},
	year={2018}
}

// facial landmark detection

@inproceedings{dong2018san,
	title={Style Aggregated Network for Facial Landmark Detection},
	author={Dong, Xuanyi and Yan, Yan and Ouyang, Wanli and Yang, Yi},
	booktitle={CVPR},
	year={2018}
}

@inproceedings{bulat2017far,
	title={How far are we from solving the 2D \& 3D Face Alignment problem? (and a dataset of 230,000 3D facial landmarks)},
	author={Bulat, Adrian and Tzimiropoulos, Georgios},
	booktitle={ICCV},
	year={2017}
}
